Hallucination Detection-Guided Preference Optimization for Clinical Summarization

Large language models (LLMs) have shown promise on summarization tasks, but they often produce hallucinations, which are unsupported or incorrect statements that limit their reliability in specialized healthcare applications. We introduce Hallucination Detection Guided Self-Refinement (HDSR), an inference-time method that leverages hallucination detectors to guide iterative summary revisions toward factual corrections. Building on this, we propose HDSR for Preference Learning (HDSR-PL), which converts detector-guided refinement trajectories into preference pairs for model finetuning. Extensive experiments show that our methods substantially reduce hallucinations for Llama and Gemma models in summarizing real-world clinical notes from MIMIC-IV-Note v2.2. For example, HDSR reduces 24% and HDSR-PL reduces 48% hallucinations in Llama-3.1-8B-Instruct. Importantly, both methods preserve summary fluency, coherence, and relevance according to human expert and LLM-Jury evaluations. Together, these results demonstrate that detection-informed refinement and preference learning offer an automated solution for improving factual faithfulness in clinical summarization.

==> 01-intro.tex <==
\section{Introduction} 

Large Language models (LLMs) have achieved strong summarization performance. However, they often generate hallucinations--content not supported by the source or inconsistent with world knowledge \citep{maynez2020FaithfulnessFactuality, ji2023SurveyHallucination, tang2023EvaluatingLarge}. Hallucinations remain prevalent even in recent LLMs, with rates of roughly 40-50\% across benchmarks such as \textsc{FaithBench} \citep{bao2025FaithBenchDiverse} indicating that factual unreliability persists despite substantial advances in scale and alignment. The challenge of hallucination becomes even more critical in clinical summarization, an emerging application area where LLMs are tasked with generating concise summaries of long patient records.

Clinical summarization supports care delivery by condensing fragmented records for provider coordination and patient communication. LLM-based systems aim to assist this process--and thereby enhance patient understanding--by easing documentation workloads that can exceed twice the time spent in direct care \citep{lee2024ProspectsAI, williams2025EvaluatingLarge}. However, despite performance comparable to clinician-written summaries \citep{veen2024AdaptedLarge}, hallucinations remain frequent, manifesting as fabricated or contextually distorted clinical statements that are difficult to detect \citep{asgari2025FrameworkAssess, kim2025MedicalHallucinations}. Because such errors can propagate into decision-making and patient dialogue, clinical summarization demands substantially stricter factual reliability than general-domain summarization.

\begin{figure*}[h]
  \centering
  \includesvg[width=\linewidth]{figs/Figure1--HM}
  \caption{\textbf{Given a clinical note, LLMs may generate fluent summaries that introduce unsupported medical claims.} Unguided self-refinement often yields stylistic improvements without correcting factual errors. Our framework uses hallucination detection signals to guide refinement toward evidence-supported revisions and couples these refined outputs with preference learning, aligning the model to prefer factually supported summaries at inference time.
}
  \label{fig:problem}
\end{figure*}

More recent work seeks to integrate feedback directly into model behavior. \SelfRefine \citep{madaan2023SelfRefineIterative} and related verification-loop methods \citep{tang2023EvaluatingLarge} iteratively critique and revise generations, improving factuality but incurring high inference cost and occasional over-editing. \SynFac \citep{mishra2024SYNFACEDITSynthetic} represents the closest line of research to ours: it generates synthetic edit feedback and trains models through preference optimization to correct hallucinations. However, its reliance on predefined error types and external edit models limits generalization and introduces additional supervision overhead.

In contrast, our framework unifies detection and preference learning within a single training objective, allowing the model to derive factual preferences directly from hallucination-detection signals—eliminating extra annotation or iterative refinement. As shown in Figure~\ref{fig:problem}, the detection signals act as guidance during self-refinement, steering the model toward fact-consistent revisions and reinforcing these preferences through optimization. \JT{Should emphasize/highlight more on the ``guidance'' effect / behavior in our framework to further articulate the intuition why our framework works. It's better if we have a (preliminary) result showing this interesting behavior}

Empirically, our approach substantially reduces hallucinations while maintaining summary quality. In particular, on MIMIC-IV clinical summarization hallucination datasets \citep{hegselmann2024DataCentricApproach}, the learned factual preferences generalize across medical note types \JT{put the most impressive numbers here for concrete results}.
These results indicate that our framework internalizes domain-specific factual alignment without added inference-time cost.


Our main contributions are as follows:
\begin{itemize}
    \item We propose a detection-informed preference learning framework that frames hallucination mitigation as preference optimization for clinical summarization.
    \item We demonstrate that factual preferences can be derived from model self-reflection, eliminating the need for manual annotation or synthetic edit feedback.
    \item We conduct comprehensive experiments on MIMIC-IV clinical summarization hallucination datasets, showing substantial factuality gains without sacrificing fluency or efficiency.
    \item We provide a detailed analysis of hallucination types, transferability, and remaining failure modes, highlighting future directions for factual alignment in medical LLMs.
\end{itemize}



==> 02-related.tex <==
\section{Related Work}
\SR{This is duplicated from the Introduction}Hallucinations, defined as content that is unsupported by the source document or contradicts known facts, remain a persistent challenge in abstractive summarization \citep{maynez2020FaithfulnessFactuality, ji2023SurveyHallucination, huang2025SurveyHallucination}. 
Despite advances in model scale, alignment, and instruction tuning, modern large language models continue to hallucinate at nontrivial rates, with recent benchmarks reporting hallucination frequencies of 40 to 50 percent across summarization tasks \citep{bao2025FaithBenchDiverse, openai2024GPT4Technical}.

Prior work has characterized hallucinations under related notions such as factual inconsistency, lack of entailment, and unsupported generation \citep{kryscinski2020EvaluatingFactual, tang2023UnderstandingFactual, lamsiyahTrustVerify}, which differ in whether hallucinations are treated primarily as evaluation artifacts or as targets for mitigation.

In clinical summarization, hallucinations are especially problematic due to the high stakes of medical decision making \citep{asgari2025FrameworkAssess, kim2025MedicalHallucinations}.

Empirical studies show that even domain adapted models frequently introduce fabricated findings, incorrect negations, or overconfident assertions that are not supported by the source record \citep{hegselmann2024DataCentricApproach, williams2025EvaluatingLarge}.

Such errors are often expressed using medically plausible terminology, making them difficult to detect without expert review \citep{fang2024UnderstandingFaithfulness, das2025HallucinationsKey}.

Consequently, clinical hallucinations are better understood as semantic misalignment at the level of medical events and attributes, including certainty and negation, rather than surface level factual errors or stylistic inconsistencies. This framing motivates mitigation approaches that explicitly reason over event level entailment to preserve clinical meaning.

Existing hallucination mitigation methods can be broadly divided into training time and inference time strategies, often combined with data curation or augmentation. At training time, one line of work focuses on pre training or continual pre training to incorporate domain knowledge or update outdated information. While such approaches can improve factuality over time, they require massive amounts of domain specific data and computational resources, making them difficult to adapt for task specific settings such as clinical summarization. More commonly, models are adapted through supervised fine tuning or parameter efficient methods such as adapters on domain specific summarization tasks \citep{veen2024AdaptedLarge, zaretsky2024GenerativeArtificial}.

However, these approaches depend on large scale, high quality reference summaries, which are costly to obtain and may themselves contain omissions or factual errors, limiting their effectiveness for hallucination mitigation \citep{hegselmann2024DataCentricApproach}.


Other training time methods attempt to directly penalize hallucinations through auxiliary loss functions or reinforcement learning based objectives. Designing loss functions that reliably capture factual faithfulness remains challenging, as existing factuality metrics often correlate weakly with clinical correctness and are sensitive to surface form rather than semantic entailment \citep{fabbri2021SummEvalReevaluating, bao2025FaithBenchDiverse, asgari2025FrameworkAssess}.

Reinforcement learning from human or AI feedback, including preference learning, auxiliary critics, and self critics, offers a more flexible alternative \citep{lee2024RLAIFVs}. However, these approaches still require carefully designed feedback signals or curated preference data, which can be difficult to scale in the clinical domain.

At inference time, a complementary set of approaches aim to reduce hallucinations without modifying model parameters. Retrieval augmented generation grounds outputs in external documents or databases, but its effectiveness depends heavily on retrieval quality. In clinical settings, retrieval errors, conflicting evidence across time, and inaccuracies in source records can propagate misleading information into generated summaries \citep{koopman2023DrChatGPT, wan2024WhatEvidence, kim2025MedicalHallucinations}.

Other inference time strategies include decoding constraints, uncertainty quantification, and self refinement through iterative feedback or reasoning \citep{madaan2023SelfRefineIterative, ji2023MitigatingHallucination}.

While self refinement can improve factuality in individual outputs, it introduces additional computational cost and can be unstable for summarization, where revisions may omit salient information or introduce new unsupported content through paraphrasing.

Across both training time and inference time approaches, data curation and augmentation play a central role. Efforts include improving the quality of domain data, generating synthetic examples with human or AI in the loop, and incorporating structured or multimodal sources such as tables, databases, or knowledge graphs. Although these strategies can enhance supervision, they do not by themselves resolve the challenge of deriving reliable, task aligned signals for factual faithfulness in clinical summarization.

Several recent studies combine self refinement with learning based alignment. \citep{ji2023MitigatingHallucination} introduce an interactive self reflection framework for medical question answering, in which models iteratively acquire knowledge and revise responses. While conceptually related, this setting differs from clinical summarization, where the primary challenge lies in retaining salient information while preserving factual and epistemic alignment. In summarization, iterative refinement can simultaneously remove important content and introduce new hallucinations, even when the revised text appears fluent.

The work most closely related to ours is \SynFac \citep{mishra2024SYNFACEDITSynthetic}, which frames hallucination mitigation in clinical summarization as a preference optimization problem. \SynFac constructs supervision by generating synthetic hallucinations based on predefined error types and training an auxiliary edit model to produce corrected summaries, which are then used for preference learning. This approach demonstrates the effectiveness of preference based objectives but relies on externally defined error taxonomies and synthetic perturbations, introducing additional modeling infrastructure and supervision overhead. In contrast, our approach derives preference signals from hallucination detection applied directly to the model’s own generations, capturing naturally occurring factual failures without predefined error schema. By integrating detection informed self refinement with preference learning into a single, self contained training pipeline, our method internalizes factual preferences at training time while avoiding inference time refinement.


==> A-datasets.tex <==
\section{Datasets}\n% Extra dataset details.\n


==> Table2.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l c c}
\toprule
\textbf{Model / Method} &
\textbf{Hallucination Count $\downarrow$} &
\textbf{LLM-as-a-Jury Average $\uparrow$} \\
\midrule
\modelheader{LLaMA-3.2-3B-Instruct}
Zeroshot & 26 & 4.28 \\
\model & 13 & 4.31 \\
\midrule

\modelheader{Gemma-3-4B-it}
Zeroshot& 15 & 4.54 \\
\model & 13 & 4.56 \\
\bottomrule
\end{tabular}
\caption{\textbf{Small-model analysis on \HalluGenDi.} Comparison of zero-shot and \modelfull (\model) for LLaMA-3.2-3B and Gemma-3-4B. \model reduces hallucination counts while maintaining comparable LLM-as-a-Jury evaluation scores.}

\label{tab:analysis_table2}
\end{table}


==> ablation_4.3.1.tex <==
\begin{table*}[htb!]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l c | c c c c}
\toprule
\multirow{2}{*}{\textbf{Model / Method}} &
\multirow{2}{*}{\makecell{\textbf{Hallucination}\\\textbf{Count} $\downarrow$}} &
\multicolumn{4}{c}{\textbf{Summary Quality Metrics}} \\
\cmidrule(lr){3-6}
& &
\textbf{Consistency}$\uparrow$ &
\textbf{Coherence}$\uparrow$ &
\textbf{Fluency}$\uparrow$ &
\textbf{Relevance}$\uparrow$ \\
\midrule

% \modelheader{GPT-5}
% Zero-shot & 36 & 3.55 & 4.73 & 4.73 & 4.08 \\
% \midrule

% \modelheader{LLaMA-3.1-8B-Instruct}
Self-Refine (No Det.) & 31 & 3.85 & 4.25 & \textbf{4.58} & \textbf{4.20} \\
\itermodel (w/MedCat) & 25 & 4.08 & \textbf{4.55} & \textbf{4.58} & 4.13 \\
\itermodel (w/MedAlign) & \textbf{22} & \textbf{4.13} & 4.48 & 4.53 & 3.95 \\
\bottomrule
\end{tabular}
\caption{\textbf{Impact of detection signal for hallucination mitigation.} Comparison between self-refinement with and without detectors on LLaMA-3.1-8B.}

\label{tab:ablation_results}
\end{table*}


==> ablation_detector.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l c | c c | c}
\toprule
\textbf{Method} &
\makecell{\textbf{Hallucination}\\\textbf{Count} $\downarrow$} &
\textbf{Relevance} &
\textbf{Consistency} &
\textbf{Length} \\
\midrule
\multicolumn{5}{l}{\textit{LLaMA-3.1-8B-Instruct}} \\
DPO (no detector) &  &  &  &  \\
DPO + MedAlign &  &  &  &  \\
DPO + MedCat &  &  &  &  \\
\midrule
\multicolumn{5}{l}{\textit{MedGemma-4B-IT}} \\
DPO (no detector) &  &  &  &  \\
DPO + MedAlign &  &  &  &  \\
DPO + MedCat &  &  &  &  \\
\bottomrule
\end{tabular}
\caption{\textbf{Detector ablation for preference learning.}
Effect of detector signal on DPO training. All settings use the same base model, training procedure, and decoding configuration; only the detector used to construct preference pairs is varied.}
\label{tab:detector_ablation}
\end{table}

==> ablation_overall.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{l c c c c c c}
\toprule
\textbf{Model Variant} &
\textbf{$\Delta$Halluc.} &
\textbf{$\Delta$Rel.} &
\textbf{$\Delta$Cons.} &
\textbf{$\Delta$Coh.} &
\textbf{$\Delta$Flu.} &
\textbf{$\Delta$Simpl.} \\
& (\%) $\downarrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$ & $\uparrow$ \\
\midrule

\modelheader{LLaMA-3.1-8B (vs.\ 0-shot)}
SFT                    & -10.52 & -0.53 & -0.46 & -0.33 & -0.19 & -0.55 \\
Self-Refine (None)     & -24.25 & +0.08 & +0.00 & -0.28 & -0.15 & -1.19 \\
Self-Refine + MedAlign & -23.49 & \textbf{+0.14} & \textbf{+0.18} & -0.15 & -0.09 & -0.95 \\
Self-Refine + MedCat   & \textbf{-30.85} & +0.06 & +0.01 & -0.34 & -0.25 & -1.15 \\
DPO + SR + MedAlign         & -5.48  & -0.01 & +0.04 & -0.04 & \textbf{+0.01} & \textbf{-0.21} \\
DPO + SR + MedCat           & -2.26  & +0.08 & +0.09 & \textbf{-0.01} & \textbf{+0.01} & -0.23 \\
\midrule

\modelheader{MedGemma-4B-IT (vs.\ 0-shot)}
SFT                    & +27.55 & -0.78 & -0.98 & -0.46 & -0.16 & \textbf{+0.18} \\
Self-Refine (None)     & \textbf{-7.44}  & -0.05 & -0.08 & -0.11 & -0.29 & -0.61 \\
Self-Refine + MedAlign & +0.07  & +0.13 & -0.08 & -0.01 & \textbf{+0.10} & +0.01 \\
Self-Refine + MedCat   & -3.67  & \textbf{+0.16} & \textbf{+0.13} & +0.00 & +0.08 & -0.05 \\
DPO + SR + MedAlign         & -1.15  & +0.11 & +0.03 & +0.04 & \textbf{+0.10} & +0.04 \\
DPO + SR + MedCat           & -0.63  & +0.10 & +0.08 & \textbf{+0.06} & +0.04 & -0.01 \\
\bottomrule
\end{tabular}
\caption{\textbf{Relative performance of adaptation methods.}
Each row reports change ($\Delta$) relative to the corresponding zero-shot
baseline for that model family. Negative $\Delta$Halluc.~indicates fewer
hallucinations (better). Values rounded to two decimals.}
\label{tab:delta_ablation}
\end{table*}


==> ablation_preference_learning.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l c c}
\toprule
\textbf{Method} &
\textbf{Detector} &
\textbf{Hallucination Rate} $\downarrow$ \\
\midrule

\multicolumn{3}{l}{\textit{LLaMA-3.1-8B-Instruct}} \\
DPO & MedAlign & -- \\
DPO & MedCAT & -- \\
DPO & None & -- \\
SALT & MedAlign & -- \\
SALT & MedCAT & -- \\
SALT & None & -- \\
\midrule

\multicolumn{3}{l}{\textit{MedGemma-4B-IT}} \\
DPO & SR + MedAlign & -- \\
DPO & SR + MedCAT & -- \\
DPO & SR & -- \\
SALT & SR + MedAlign & -- \\
SALT & SR + MedCAT & -- \\
SALT & SR & -- \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation on detector choice and preference learning objective.}
We compare DPO and SALT under different hallucination detectors.
Lower hallucination rate indicates better faithfulness.}
\label{tab:ablation_detector_objective}
\end{table}

==> ablation_self_refinement_preference_learning.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l c c}
\toprule
\textbf{Training Strategy} &
\textbf{Detector} &
\textbf{Hallucination Rate} $\downarrow$ \\
\midrule

\multicolumn{3}{l}{\textit{LLaMA-3.1-8B-Instruct}} \\
Self-Refinement & MedAlign & -- \\
Self-Refinement & MedCAT & -- \\
Self-Refinement & None & -- \\
Preference Learning (DPO) & MedAlign & -- \\
Preference Learning (DPO) & MedCAT & -- \\
Preference Learning (DPO) & None & -- \\
\midrule

\multicolumn{3}{l}{\textit{MedGemma-4B-IT}} \\
Self-Refinement & MedAlign & -- \\
Self-Refinement & MedCAT & -- \\
Self-Refinement & None & -- \\
Preference Learning (DPO) & MedAlign & -- \\
Preference Learning (DPO) & MedCAT & -- \\
Preference Learning (DPO) & None & -- \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison between self-refinement and preference learning.}
Preference learning consistently achieves lower hallucination rates across detectors and base models.}
\label{tab:ablation_self_refine}
\end{table}

==> analysis_hallucination_counts.tex <==
% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
%     \hline
%         \textbf{Dataset / Model} & \textbf{Unsupported Condition} & \textbf{Unsupported Procedure} & \textbf{Unsupported Medication} & \textbf{Unsupported Time} & \textbf{Unsupported Location} & \textbf{Unsupported Number} & \textbf{Unsupported Name} & \textbf{Unsupported Word} & \textbf{Unsupported Other} & \textbf{Contradicted Fact} & \textbf{Incorrect Fact} & \textbf{Total} \\ \hline
%         GPT-4.1 0-shot & 3 & 0 & 0 & 1 & 2 & 0 & 0 & 0 & 1 & 3 & 0 & 10 \\ \hline
%         GPT-5 0-shot & 7 & 4 & 4 & 3 & 4 & 1 & 2 & 1 & 0 & 10 & 0 & 36 \\ \hline
%         Llama-3.1-8B-Instruct 0-shot & 8 & 2 & 1 & 3 & 4 & 0 & 1 & 2 & 0 & 8 & 0 & 29 \\ \hline
%         MedGemma-4b-it 0-shot & 0 & 2 & 1 & 2 & 0 & 0 & 1 & 2 & 1 & 5 & 0 & 14 \\ \hline
%         ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
%         Llama-3.1-8B-Instruct 0-shot & 8 & 2 & 1 & 3 & 4 & 0 & 1 & 2 & 0 & 8 & 0 & 29 \\ \hline
%         Llama SFT & 15 & 11 & 8 & 3 & 6 & 0 & 3 & 3 & 1 & 7 & 0 & 57 \\ \hline
%         Llama Self-Refine & 10 & 2 & 6 & 2 & 3 & 3 & 1 & 1 & 1 & 2 & 0 & 31 \\ \hline
%         Llama Self-Refine w/ MedCat & 7 & 1 & 3 & 4 & 3 & 2 & 2 & 2 & 0 & 1 & 0 & 25 \\ \hline
%         Llama Self-Refine w/ MedAlign & 4 & 2 & 1 & 3 & 3 & 1 & 1 & 0 & 2 & 5 & 0 & 22 \\ \hline
%         Llama Self-Refine DPO (best; MedCat) & 3 & 1 & 0 & 1 & 2 & 0 & 0 & 0 & 0 & 8 & 0 & 15 \\ \hline
%         ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
%         MedGemma-4b-it 0-shot & 0 & 2 & 1 & 2 & 0 & 0 & 1 & 2 & 1 & 5 & 0 & 14 \\ \hline
%         MedGemma SFT & 40 & 22 & 27 & 17 & 10 & 4 & 6 & 25 & 25 & 18 & 1 & 195 \\ \hline
%         MedGemma Self-Refine & 5 & 0 & 4 & 2 & 0 & 2 & 0 & 3 & 2 & 11 & 0 & 29 \\ \hline
%         MedGemma Self-Refine w/ MedCat & 3 & 2 & 2 & 1 & 3 & 0 & 0 & 0 & 1 & 9 & 0 & 21 \\ \hline
%         MedGemma Self-Refine w/ MedAlign & 3 & 1 & 1 & 3 & 4 & 0 & 1 & 0 & 0 & 10 & 0 & 23 \\ \hline
%         MedGemma Self-Refine DPO (best; MedCat) & 3 & 0 & 2 & 2 & 1 & 0 & 1 & 1 & 0 & 8 & 0 & 18 \\ \hline
%         ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
%         Llama Self-Refine w/ MedCat DPO & 3 & 1 & 0 & 1 & 2 & 0 & 0 & 0 & 0 & 8 & 0 & 15 \\ \hline
%         Llama Self-Refine w/ MedAlign DPO & 3 & 2 & 0 & 2 & 2 & 0 & 1 & 1 & 0 & 5 & 0 & 16 \\ \hline
%         MedGemma Self-Refine w/ MedCat DPO & 3 & 0 & 2 & 2 & 1 & 0 & 1 & 1 & 0 & 8 & 0 & 18 \\ \hline
%         MedGemma Self-Refine w/ MedAlign DPO & 2 & 1 & 1 & 2 & 1 & 0 & 0 & 2 & 0 & 11 & 0 & 20 \\ \hline
%     \end{tabular}
%     \label{tab:analysis}
% \end{table}

\begin{table*}[htb!]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}

\begin{tabular}{lrrrrrrrrrrr}
\toprule
\textbf{Model} &
\rotatebox{90}{\textbf{Unsupported Condition}} &
\rotatebox{90}{\textbf{Unsupported Procedure}} &
\rotatebox{90}{\textbf{Unsupported Medication}} &
\rotatebox{90}{\textbf{Unsupported Time}} &
\rotatebox{90}{\textbf{Unsupported Location}} &
\rotatebox{90}{\textbf{Unsupported Number}} &
\rotatebox{90}{\textbf{Unsupported Name}} &
\rotatebox{90}{\textbf{Unsupported Word}} &
\rotatebox{90}{\textbf{Unsupported Other}} &
\rotatebox{90}{\textbf{Contradicted Fact}} &
\rotatebox{90}{\textbf{Incorrect Fact}} \\
\midrule

% \multicolumn{13}{l}{\emph{Zero-shot baselines}} \\
% GPT-4.1 (0-shot) & 3 & 0 & 0 & 1 & 2 & 0 & 0 & 0 & 1 & 3 & 0 & 10 \\
% GPT-5 (0-shot)   & 7 & 4 & 4 & 3 & 4 & 1 & 2 & 1 & 0 & 10 & 0 & 36 \\
% LLaMA-3.1-8B-Instruct (0-shot) & 8 & 2 & 1 & 3 & 4 & 0 & 1 & 2 & 0 & 8 & 0 & 29 \\
% MedGemma-4B-IT (0-shot) & 0 & 2 & 1 & 2 & 0 & 0 & 1 & 2 & 1 & 5 & 0 & 14 \\

% \midrule
\multicolumn{13}{l}{\emph{LLaMA-3.1-8B-Instruct}} \\
Prompting & 8 & 2 & 1 & 3 & 4 & 0 & 1 & 2 & 0 & 8 & 0\\
SFT & 15 & 11 & 8 & 3 & 6 & 0 & 3 & 3 & 1 & 7 & 0\\
Self-Refine (No Det.) & 10 & 2 & 6 & 2 & 3 & 3 & 1 & 1 & 1 & 2 & 0\\
\itermodel (w/MedCat) & 7 & 1 & 3 & 4 & 3 & 2 & 2 & 2 & 0 & 1 & 0\\
\itermodel (w/MedAlign) & 4 & 2 & 1 & 3 & 3 & 1 & 1 & 0 & 2 & 5 & 0\\
\model (best; MedCat) & 3 & 1 & 0 & 1 & 2 & 0 & 0 & 0 & 0 & 8 & 0\\

% \midrule
% \multicolumn{13}{l}{\emph{MedGemma variants}} \\
% Prompted & 0 & 2 & 1 & 2 & 0 & 0 & 1 & 2 & 1 & 5 & 0 & 14 \\
% SFT & 40 & 22 & 27 & 17 & 10 & 4 & 6 & 25 & 25 & 18 & 1 & 195 \\
% Self-Refine & 5 & 0 & 4 & 2 & 0 & 2 & 0 & 3 & 2 & 11 & 0 & 29 \\
% Self-Refine w/ MedCat & 3 & 2 & 2 & 1 & 3 & 0 & 0 & 0 & 1 & 9 & 0 & 21 \\
% Self-Refine w/ MedAlign & 3 & 1 & 1 & 3 & 4 & 0 & 1 & 0 & 0 & 10 & 0 & 23 \\
% Self-Refine DPO (best; MedCat) & 3 & 0 & 2 & 2 & 1 & 0 & 1 & 1 & 0 & 8 & 0 & 18 \\

\bottomrule
\end{tabular}

\caption{Distribution of hallucination error types across models.}
\label{tab:analysis}
\end{table*}

% \begin{table}[t]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.05}

% % If it still doesn’t fit, slightly reduce \tabcolsep or switch \scriptsize -> \tiny.
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lrrrrrrrrrrr}
% \toprule
% \textbf{Model} &
% \rotatebox{90}{\textbf{Unsupported Condition}} &
% \rotatebox{90}{\textbf{Unsupported Procedure}} &
% \rotatebox{90}{\textbf{Unsupported Medication}} &
% \rotatebox{90}{\textbf{Unsupported Time}} &
% \rotatebox{90}{\textbf{Unsupported Location}} &
% \rotatebox{90}{\textbf{Unsupported Number}} &
% \rotatebox{90}{\textbf{Unsupported Name}} &
% \rotatebox{90}{\textbf{Unsupported Word}} &
% \rotatebox{90}{\textbf{Unsupported Other}} &
% \rotatebox{90}{\textbf{Contradicted Fact}} &
% \rotatebox{90}{\textbf{Incorrect Fact}} \\
% \midrule

% \multicolumn{12}{l}{\emph{LLaMA-3.1-8B-Instruct}} \\
% Prompting &
% \heatcell{8} & \heatcell{2} & \heatcell{1} & \heatcell{3} & \heatcell{4} &
% \heatcell{0} & \heatcell{1} & \heatcell{2} & \heatcell{0} & \heatcell{8} & \heatcell{0} \\
% SFT &
% \heatcell{15} & \heatcell{11} & \heatcell{8} & \heatcell{3} & \heatcell{6} &
% \heatcell{0} & \heatcell{3} & \heatcell{3} & \heatcell{1} & \heatcell{7} & \heatcell{0} \\
% Self-Refine (No Det.) &
% \heatcell{10} & \heatcell{2} & \heatcell{6} & \heatcell{2} & \heatcell{3} &
% \heatcell{3} & \heatcell{1} & \heatcell{1} & \heatcell{1} & \heatcell{2} & \heatcell{0} \\
% \itermodel\ (w/MedCat) &
% \heatcell{7} & \heatcell{1} & \heatcell{3} & \heatcell{4} & \heatcell{3} &
% \heatcell{2} & \heatcell{2} & \heatcell{2} & \heatcell{0} & \heatcell{1} & \heatcell{0} \\
% \itermodel\ (w/MedAlign) &
% \heatcell{4} & \heatcell{2} & \heatcell{1} & \heatcell{3} & \heatcell{3} &
% \heatcell{1} & \heatcell{1} & \heatcell{0} & \heatcell{2} & \heatcell{5} & \heatcell{0} \\
% \model\ (best; MedCat) &
% \heatcell{3} & \heatcell{1} & \heatcell{0} & \heatcell{1} & \heatcell{2} &
% \heatcell{0} & \heatcell{0} & \heatcell{0} & \heatcell{0} & \heatcell{8} & \heatcell{0} \\

% \bottomrule
% \end{tabular}%
% }

% \caption{Distribution of hallucination error types. Cell shading uses a colorblind-safe blue--orange scale (low to high).}
% \label{tab:analysis_onecol}
% \end{table}

==> summarization_metrics.tex <==
% {"rouge1": 37.01, "rouge2": 11.59, "rouge3": 5.39, "rouge4": 2.41, "rougeL": 22.56, "words": 146.35, "bert_score": 86.81, "bert_score_deberta-large": 61.49, "sari": 44.1, "file": "dpo-medalign-llama-3.1-8b-instruct-hallucinations_generated_di.jsonl"}

% {"rouge1": 36.9, "rouge2": 11.39, "rouge3": 5.26, "rouge4": 2.16, "rougeL": 23.48, "words": 95.75, "bert_score": 86.71, "bert_score_deberta-large": 61.63, "sari": 41.1, "file": "dpo-medalign-medgemma-4b-it-hallucinations_generated_di.jsonl"}

% {"rouge1": 37.91, "rouge2": 12.02, "rouge3": 5.28, "rouge4": 2.02, "rougeL": 23.73, "words": 144.7, "bert_score": 86.68, "bert_score_deberta-large": 61.03, "sari": 43.57, "file": "dpo-medcat-llama-3.1-8b-instruct-hallucinations_generated_di.jsonl"}

% {"rouge1": 36.79, "rouge2": 11.17, "rouge3": 4.68, "rouge4": 1.64, "rougeL": 23.64, "words": 97.9, "bert_score": 86.56, "bert_score_deberta-large": 60.49, "sari": 41.36, "file": "dpo-medcat-medgemma-4b-it-hallucinations_generated_di.jsonl"}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l c c c c c c c c}
\toprule
\textbf{Model / Variant} &
\textbf{R1 $\uparrow$} &
\textbf{R2 $\uparrow$} &
\textbf{R3 $\uparrow$} &
\textbf{R4 $\uparrow$} &
\textbf{RL $\uparrow$} &
\textbf{Words $\downarrow$} &
\textbf{BERTScore $\uparrow$} &
\textbf{SARI $\uparrow$} \\
\midrule

\textit{LLaMA-3.1-8B-Instruct} \\
\quad w/ MedAlign (SR + DPO) & 37.01 & 11.59 & \textbf{5.39} & \textbf{2.41} & 22.56 & 146.35 & \textbf{86.81} & \textbf{44.10} \\
\quad w/ MedCAT (SR + DPO)   & \textbf{37.91} & \textbf{12.02} & 5.28 & 2.02 & \textbf{23.73 }& \textbf{144.70} & 86.68 & 43.57 \\
\midrule

\textit{MedGemma-4B-IT} \\
\quad w/ MedAlign (SR + DPO) & \textbf{36.90 }& \textbf{11.39} & \textbf{5.26} & \textbf{2.16} & 23.48 & 95.75 & \textbf{86.71} & 41.10 \\
\quad w/ MedCAT (SR + DPO)   & 36.79 & 11.17 & 4.68 & 1.64 & \textbf{23.64} & \textbf{97.90} & 86.56 & \textbf{41.36} \\
\bottomrule
\end{tabular}
\caption{\textbf{Summarization metrics on HALLUCINATIONS-GENERATED-DI} for model variants grouped by base model.}
\label{tab:summarization_metrics}
\end{table*}
